FUSE-ing Language Models: Zero-Shot Adapter Discovery for Prompt Optimization Across Tokenizers

The widespread use of large language models has resulted in a multitude of tokenizers and embedding spaces, making knowledge transfer in prompt discovery tasks difficult. In this work, we propose FUSE (Flexible Unification of Semantic Embeddings), an inexpensive approach to approximating an adapter layer that maps from one model's textual embedding space to another, even across different tokenizers. We introduce a third-order tensor-based representation of a model's embedding space that aligns semantic embeddings that have been split apart by different tokenizers, and use this representation to derive an approximation of the gradient of one model's outputs with respect to another model's embedding space. We show the efficacy of our approach via multi-objective optimization over vision-language and causal language models for image captioning and sentiment-based image captioning.

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

Before going into detail on our approach, we first introduce the necessary notation. Throughout this work, we denote scalars, vectors, matrices, and tensors as lowercase, $a$, bolded lowercase $\vect{a}$, uppercase $A$, and as uppercase with a tilde $\tilde{A}$, respectively.

\subsection{Language Model Embeddings}

Given a string, a tokenizer maps this string to a set of tokens, $\vect{t} \in \{0, ..., |V|\}^{s}$, where $s$ is the length of the tokenized string and $|V|$ are the number of unique tokens in the tokenizer. A language model then applies a mapping $\mathcal{E}: \{0, ..., |V|\}^{s} \rightarrow \mathcal{R}^{s \times d}$ that indexes these tokens across a discrete set of embeddings, mapping each token to a unique $d$-dimensional embedding, $E \in \mathbb{R}^{s \times d}$. 

Equivalently, let the tokens be a one-hot encoding, $X \in \{0,1\}^{s \times |V|}$ and $V$ the codomain of $\mathcal{E}$, in this case, the embeddings are expressed as $E = X V$. Here, we call $V$ the vocabulary of a model, and $V_{i}$ the vocabulary of a particular model. In this work, we are primarily concerned with the inputs to a language model, rather than their outputs. Thus, we leave the details of the models as imprecise. 

